Clean Code, Better Models: Enhancing LLM Performance with Smell-Cleaned Dataset

The Large Language Models (LLMs) have demonstrated great potential in code-related tasks. However, most research focuses on improving the output quality of LLMs (e.g., correctness), and less attention has been paid to the LLM input (e.g., the training code quality). Given that code smells are widely existed in practice and can negatively impact software maintainability and readability, this study takes the first systematic research to assess and improve dataset quality in terms of code smells. In this work, we first conduct a preliminary study to explore the presence of code smells in a popular benchmark dataset (i.e., CodeSearchNet-Python}) and evaluate the output of several popular LLMs (i.e., DeepSeek-Coder, CodeLlama, and MagiCoder), revealing that code smell issues extensively exist in LLM's input (e.g., benchmark dataset) and output (e.g., generated code). We then conduct our systematic research by taking three main steps: Firstly, we propose an LLM-based code smell cleaning tool, named SmellCC, which automatically refactors and removes code smells. To evaluate the correctness of the code refactoring, we construct a test set of 50 repositories sourced from the CodeSearchNet-Python benchmark for functional testing. Then we apply our curated smell-cleaned dataset to fine-tune two LLMs (i.e., DeepSeek-V2 and Qwen-Coder) to explore their potential for generating high-quality code. Thirdly, we investigate the impact of code smells on two downstream tasks: code completion and code search. Lastly, we derive several actionable implications for software engineering researchers and industry practitioners from our findings.

==> 6-User_Study.tex <==
\section{USER STUDY} 
In this study, one of the core contributions is that we developed an LLM-based code smell cleaning tool, \tool, for addressing different code smell issues in the training set and curating a smell-cleaned dataset. 
To further understand how effective our \tool for cleaning code smells is in practice, we conducted a user study to investigate how developers perceive the smell cleaning results and whether they can improve the software quality and maintainability. 
% In this study, % we focus on constructing a high-quality training dataset using LLMs and further enhancing their performance by fine-tuning with a cleaned dataset. 
% The critical aspect is how effectively the LLM can remove code smells to improve the dataset's overall quality. 
% While we have evaluated the LLM's ability to eliminate code smells using static analysis tools and manual validation, we also conducted a user study to avoid knowledge bias and further evaluate the quality of the cleaned dataset.


\begin{figure} % [htbp]
    \centering
    \includegraphics[width=0.95\textwidth]{user-study-questions.pdf} %questions.pdf
    \caption{The Question for The Original Code and Refactored Code}
    \label{fig:question}
\end{figure}


\subsection{User Study Setup}
To conduct the user study, we designed 5 questionnaires. 
Each questionnaire contains 10 code smell instances (each category with one instance), each code smell contains a pair of code snippets, the original code with code smells and the cleaned code (potentially) without code smells. 
We first briefly introduce the code smell to the evaluator and then ask the evaluator to answer the following questions: 
(1) \textit{Do you think the functional correctness of these two code samples is consistent?} 
(2) \textit{Do you think the code smell of this type is addressed?} 
(3) \textit{By comparing the code, do you think the refactoring improves the code quality?} 
(4) \textit{Please rate the original code in terms of readability and maintainability: (from 1 to 5, 5 is the best).} 
(5) \textit{Please rate the refactored code in terms of readability and maintainability: (from 1 to 5, 5 is the best).} 
An example of a code smell instance in our user study is demonstrated in Fig.~\ref{fig:question}. 
We invite 20 participants for this user study. 
Each questionnaire was sent to four evaluators to perform the human evaluation. 
In other words, each code smell instance has five instances, and each instance was evaluated by four participants independently. 
We collected 200 responses (10 categories x 5 instances x 4 participants) for this study. 
Before filling the questionnaires, we collected the background of the 20 participants. 
The participants are developers in computer science or software engineering majors, have Python programming experience ranging from two years to ten years. 
75\% of them are familiar with code smells and resolved code smell issues in their daily development. 

% We conduct a controlled experiment to evaluate the quality of the cleaned dataset on readability and maintainability. Participants were assigned to read code either with
% or without code smell issues. The experiment involved 20 developers with programming experience ranging from two to ten years in Python.

% Before the experiment, we learned about the participants’ familiarity and experience of handling code smells through a pre-study survey. 75\% of them are familiar with code smell and have resolved code smell issues. Most of them deal with code smell by refactoring the code smell by themselves (9/15) or automated tools (7/15).
% We randomly split 20 students into five groups and assigned different codes to each group.

% For the experiment, we design 50 questions by randomly selecting 5 code smell instances for each category from CodeSearchNet. For each category of code smell, we ensure that selected code smell instances are from different GitHub projects. Fig.~\ref{fig:question} gives an example of the chain-comparison provided to the experimental group with the smell code and the corresponding smell-well code. We collect 200 answers (10 questions×20 participants) for the study.

\begin{table} % [h]
\setlength{\abovecaptionskip}{0pt}
    \caption{User Study Results}   
    \label{tab:user study}  
    \centering 
    \scalebox{0.7}{
    \begin{tabular}{l r r r c c}  
      \specialrule{1pt}{1pt}{1pt}  
      Type & Functional Consistency & Code Smell Elimination & Quality Improvement & Readability & Maintainability\\  
      \hline  
      \textit{Commented Code} &  17/20 (85\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.85,0.2);
        \fill[white] (0.85,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      17/20 (85\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.85,0.2);
        \fill[white] (0.85,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 3.00 $\rightarrow$ 4.00 & 2.95$\rightarrow$ 4.35
      \\  
            \textit{Naming Convention} &  19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      17/20 (85\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.85,0.2);
        \fill[white] (0.85,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 2.90$\rightarrow$ 4.00 &	2.85$\rightarrow$ 4.10
      \\  
        \textit{Empty Nested Code Blocks}  &  12/20 (60\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.6,0.2);
        \fill[white] (0.6,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 3.05 $\rightarrow$ 4.15& 2.45$\rightarrow$ 4.20

      \\  
        \textit{Collapsible if Statements} &  19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      &2.60 $\rightarrow$4.30	&2.75 $\rightarrow$4.25

      \\  
       \textit{Long Parameter List}&  16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}
      & 2.50 $\rightarrow$4.05	&2.50 $\rightarrow$4.05
      \\  
      \textit{High Cognitive Complexity} &  16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}  & 
      15/20 (75\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.75,0.2);
        \fill[white] (0.75,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}  & 
    16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}
      & 2.50 $\rightarrow$4.05 &2.35	$\rightarrow$4.25
      \\  
       \textit{Dead Code} &  18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      20/20 (100\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (1,0.2);
        \fill[white] (1,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    20/20 (100\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (1,0.2);
        \fill[white] (1,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 2.75$\rightarrow$4.00	&2.50 $\rightarrow$4.35
      \\  
      \textit{Self-assigned Variables} &   16/20 (80\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.8,0.2);
        \fill[white] (0.8,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
   19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 2.60 $\rightarrow$4.30 &	2.50$\rightarrow$4.45

      \\  
            \textit{Identical Expressions} &  17/20 (85\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.85,0.2);
        \fill[white] (0.85,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
      20/20 (100\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (1,0.2);
        \fill[white] (1,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
    20/20 (100\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (1,0.2);
        \fill[white] (1,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}
      &2.50$\rightarrow$4.10 & 2.35$\rightarrow$	4.50


      \\  
            \textit{Return and Yield} &  18/20 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
     19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}  & 
    19/20 (95\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.95,0.2);
        \fill[white] (0.95,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 2.85$\rightarrow$3.95 &	2.50$\rightarrow$4.25\\
    \hline  
    All & 168/200 (84\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.84,0.2);
        \fill[white] (0.84,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} & 
     182/200 (91\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.91,0.2);
        \fill[white] (0.91,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture}  & 
    180/200 (90\%)
      \begin{tikzpicture}
        \fill[black] (0,0) rectangle (0.9,0.2);
        \fill[white] (0.9,0) rectangle (1,0.2);
        \draw (0,0) rectangle (1,0.2);
      \end{tikzpicture} 
      & 2.73$\rightarrow$4.09 &	2.57$\rightarrow$4.28
      \\  
      \specialrule{1pt}{1pt}{1pt}  
    \end{tabular}  
    }
  \end{table}

  
\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{readability.pdf}
        \caption{Readability Comparison of Original and Refactored Code}
        \label{fig:readability}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{maintainability.pdf}
        \caption{Maintainability Comparison of Original and Refactored Code}
        \label{fig:maintainability}
    \end{subfigure}
    \begin{minipage}{\textwidth}
    \footnotesize
    % NC: \textit{Naming Convention}, HCC: \textit{High Cognitive Complexity}, LM: \textit{Long Method}, ENCB: \textit{Empty Nested Code Blocks}, DC: \textit{Dead Code}, SAV: \textit{Self-assigned Variables}, CC: \textit{Commented Code}, CIS: \textit{Collapsible if Statements}, IE: \textit{Identical Expressions}, RY: \textit{Return and Yield}.
\end{minipage}
    \caption{Readability and Maintainability Comparison}
    \label{fig:readability_maintainability}
\end{figure}


\subsection{User Study Results}
Table~\ref{tab:user study} illustrated our user study experimental results. 
From the table, we can see that: 
(1) In general, we found that participants agreed that most of the refactored code effectively eliminates code smells while maintaining functional consistency and enhancing code quality. 
For example, 84\% developers consider the functionality of the code before and after code refactoring is consistent, 91\% evaluators agree that the code smell is cleaned by our tool after refactoring, 90\% developers think the quality of the code is improved after addressing the corresponding code smell.
% For example, one participant said, "\textit{The refactored code is shorter and well-formatted, I think it is easier to read and understand.}"
(2) Regarding specific code smells, the performance of our tool is still suboptimal. 
For example, we observed that refactoring \textit{Empty Nested Code Blocks} may impact functional consistency. 
Specifically, 40\% (8/20) of participants expressed concerns regarding potential functionality changes after refactoring. 
We had a short discussion with these participants after they completed the questionnaire. 
Some participants believed that the condition checks within \textit{Empty Nested Code Blocks} serve a meaningful purpose and should not be removed. For instance, one participant said, "\textit{The condition check is useful for verifying values during debugging. So I think directly removing the condition check will change the functionality.}"

Fig.~\ref{fig:readability_maintainability} shows the readability and maintainability score distributions for the original code and refactored code. 
% We can find most participants vote higher scores for refactored code in terms of both readability and maintainability. 
The readability and maintainability of all ten code smells are improved after code refactoring. 
Specifically, the overall readability score increased 51.3\% after refactoring. 
Similarly, the maintainability score increased 66.3\% after refactoring. 
Regarding specific code smell instances, some developers had different opinions. For example, about \textit{Long Parameter List} issue, one participant said, ``\textit{I don't think splitting a long method into several smaller methods improves code quality. it actually makes understanding the logic more challenging across multiple methods and complicates parameter passing.}'' 
Additionally, for the \textit{Commented Code} issue, one participant said, ``\textit{The commented code involves log-related code, so I think removing such code will reduce the maintainability.}''

In the last, we asked participants two open questions regarding their attitudes toward code smells: \textbf{Do you think it is necessary to clean code smells by refactoring?} and \textbf{Will you use LLMs for addressing code smells in daily work?} 
Most participants gave positive feedback on these two questions.
For instance, one participant mentioned, ``\textit{In the past, I preferred to ignore code smells until they caused bugs, as manually refactoring is time-consuming. In the future, I will consider using LLMs to fix these code smells when they occur.}" 
However, one participant felt that code refactoring was unnecessary, stating that ``\textit{I think refactoring a code snippet is not important, but refactoring the entire software system is crucial. 
But LLMs still lack the capability in my point of view.}" 
Additionally, a few participants were hesitant to use LLMs for code refactoring. 
As one participant pointed out, ``\textit{I don’t want to verify the correctness of refactored code generated by LLMs.}''
